Proof mining in metric fixed point theory and ergodic theory

In this survey we present some recent applications of proof mining to the fixed point theory of (asymptotically) nonexpansive mappings and to the metastability (in the sense of Terence Tao) of ergodic averages in uniformly convex Banach spaces.

==> temp.tex <==


\begin{denseBibitem}{Goe02} 
K. Goebel, Concise course on fixed point theory, Yokohama Publishers, Yokohama, 2002.
\end{denseBibitem}

\begin{denseBibitem}{Koh98a}
U. Kohlenbach, Proof theory and computational analysis, Electronic Notes in Theoretical Computer Science 13 (1998), 124--158.
\end{denseBibitem}

\begin{denseBibitem}{Koh08} 
U. Kohlenbach, Effective uniform bounds from proofs in abstract functional analysis, in: 
B. Cooper, B. Loewe, A. Sorbi, (eds.), New Computational Paradigms: Changing Conceptions of What is Computable, Springer-Verlag, New York, 2008,  223--258. 
\end{denseBibitem}


\begin{denseBibitem}{Liu95}
L.-S. Liu,  Ishikawa and Mann iterative process with errors for nonlinear strongly accretive mappings in Banach spaces, J. Math. Anal. Appl. 194 (1995), 114-125.
\end{denseBibitem}


\begin{denseBibitem}{Qih01} 
L. Qihou, Iteration sequences for asymptotically quasi-nonexpansive mappings with error member, J. Math. Anal. Appl. 259 (2001), 18--24. 
\end{denseBibitem}

\begin{denseBibitem}{Qih02} 
L. Qihou, Iteration sequences for asymptotically quasi-nonexpansive mapping with an error member of uniform convex
Banach space, J. Math. Anal. Appl. 266 (2002), 468--471. 
\end{denseBibitem}


\begin{denseBibitem}{Rei82}
S. Reich, Some problems and results in fixed point theory, in: S.P. Singh, S. Thomeier, B. Watson (eds.), Topological methods in nonlinear functional analysis. Proceedings of the special session on fixed point theory and applications held during the 86th summer meeting of the American Mathematical Society at the University of Toronto, Toronto, Ont., August 21-26, 1982, Contemp. Math. 21, Amer. Math. Soc., Providence, RI, 1983, 179--187.
\end{denseBibitem}
